Medley2K: A Dataset of Medley Transitions

The automatic generation of medleys, i.e., musical pieces formed by different songs concatenated via smooth transitions, is not well studied in the current literature. To facilitate research on this topic, we make available a dataset called Medley2K that consists of 2,000 medleys and 7,712 labeled transitions. Our dataset features a rich variety of song transitions across different music genres. We provide a detailed description of this dataset and validate it by training a state-of-the-art generative model in the task of generating transitions between songs.

==> chapters/ch01-introduction.tex <==
\section{Introduction}

Our contributions are as follows:

\begin{itemize}
    \item dataset consisting of medley transitions marked, nonspecific dataset, rich variety, various beats.
    \item other way of encode held notes in piano roll
    \item music inpainting model to generate polyphonic music (rewrite)
    \item evaluation of performance of different encoding models and n voice music inpaintings over 4 bars.
    (rewrite to: Thorough experimental evaluations examine and validate the efficacy of the porposed model)
    \item evaluation metric based on beats / pitches in addition to loss, loss does not directly map to good music.
\end{itemize}

\subsection{Medley}
A Medley is an arrangement of different Melodies.
This arrangement may span several songs, genres, epochs, and composers.
%I still have to put this text somewhere
All songs are licensed as shareable, while only a subset is usable for commercial use.

==> chapters/ch02-related-work.tex <==
\section{Related Work}
This entire section may take a few days
\subsection{Dataset}
While there exists a variety of midi related datasets, this is to our best knowledge the first and only Medley dataset.
This dataset should not be confused with MedleyDB \cite{MedleyDB}, which focuses on multi-track music. An extensive list of music dataset can be found at \emph{https://ismir.net/resources/datasets}
\subsection{Transition Generation}
Related to Transition Generation(TG) for music is the field of Music Inpainting. Music Inpainting is the task of restoring an blank sub piece of music. This is in contrast to TG which fills a gap of music between two heterogeneous contexts, to make a reasonable guess from how to transition from one song to the next.
\subsection{Data Representation}
A variety of data representations has been chosen to represent music for Deep Learning.
Among the well known representation forms is the one proposed by Hadjeres et al. \cite{datarepresentation}.\\
A particularity of this representation is the representation of held notes,
it is represented using a special symbol which stands for held.
\subsection{Automatic music evaluation metrics}
While music generation using Deep Learning is a common topic, its evaluation remains mostly confined to user studies.
These user studies are expensive and do not offer immediate feedback for the developers.\\
Therefore, a set of automatic metrics which steer the development process would be desirable \cite{musicevalwhylimit}, a set of ideas for candidates has been proposed by de Freitas et al. \cite{musicevalideas}.
The concrete implementation of such metrics can be mostly found in the field of evolutionary computation \cite{evolutionaryComputation}.
However there they are mostly used as fitness functions and are directly used for the optimisation process.


==> chapters/ch03-dataset.tex <==
\section{Dataset}
We present a new dataset Medley2k.
The dataset consist of a set of 10'270 Transition Points(TP) that have been labeled.
A TP is a specific point in time at which a song in a Medley transitions from one song to the next.
We found in our work that Medley composers mostly make their transitions happen at the start of a bar.
Therefor the TP we labeled in this work will always be at the start of a new bar.
The dataset refers to a collection of 1978 human-curated songs downloaded from musescore.com.
Our dataset contains Medleys made by a variety of composers and genres.
For each song 4 files are present, a PDF containing the sheet music, a midi file containing the song, an MXL containing the XML that makes up the music sheet and a JSON file containing additional information for the song.\\
\subsection{Labeling}
    \label{sub:datasetMetrics}

To Label the transitions we use an automatic approach.
We decided to do so, since the number of songs was too extensive to label manually, and an evaluation suggested that labels generated by non-composers were not precise.
The TP in this collection do not represent all transitions that exist in the dataset.\\
We discovered that the annotation given by the composer in the sheet music is the most reliable data source, we used this method in contrast to other information present such as tempo and key-signature changes.
Often composers annotate the song which the transitions lead to the top of the first voice, as shown in figure \ref{dataset:ti}
\begin{figure}[!htb]
\centering
    \includegraphics[width=0.3\textwidth]{img/ds_transitionindicator.png}
    \caption{Transition indicator labeled by the composer}
      \label{dataset:ti}
\end{figure}
We extract this information through the MXL file, which contains the complete structural information to build the sheet music PDF.\\
To make the labels more precise we removed unique characters such as numbers, and specific music symbols such as \quarternote.
Additionally, we removed a list of 150 common words that are used at such positions in sheet music e.g. vivante, allegro and solo.
After this process, we are left with the presented selection of transitions.
A manual validation of 205 randomly selected transitions has been conducted, the results can be seen in table \ref{dataset:val}
\begin{table}[]
\begin{tabular}{l|l|l|l}
\cline{2-3}
                                      & True Positive & True Negative    \\ \cline{1-3}
\multicolumn{1}{|l|}{Predicted True}  & 117           & 12             \\ \cline{1-3}
\multicolumn{1}{|l|}{Predicted False} & 88            & 4370    \\ \cline{1-3}
\end{tabular}
    \caption{Validation of Labeling Process}
      \label{dataset:val}
\end{table}
As we can see the Precision is at 90.70\%, and the Recall is at 57.07\%. This is what we were aiming for, since we mostly operate on the Positives. Therefore having a False Positive is more costly than loosing a few transitions in the process.\\
To ensure vivid transitions we additionally provide for each transition a set of metrics.
This set of metrics is concerned with how many pitches start in the bars surrounding the TP.
A qualitative description of these metrics:
\begin{itemize}
    \item Transition time, the time in seconds in the MIDI the TP occurs at
    \item Transition bar, bar in the music sheet it occurs at
    \item Transition bar with offset, bar in the midi file the TP occurs at (accounting for repetition signs) 
    \item Amount of notes, notes played around the TP plus a small epsilon
    \item Notes starting in various half bars around the transition
\end{itemize}






==> chapters/ch035-datarepresentation.tex <==
\section{Data representation}
I order to feed a midi into a Deep Learning Model one needs to restructure it into a form it can understand.
In this work we use a variation of the encoding proposed by Hadjeres et al. \cite{datarepresentation}\\
A bar is made up in our work of 16 pitches, i.e. we used a precision of 1/16 notes to convert each of our voices into a matrix.
A Transition is a combination of 12 consecutive bars, where the first 4 bars are referred to as the past context, the middle 4 bars are referred to as the target, followed by the final 4 bars referred to as the future context as illustrated in figure \ref{dataset:trans}.
Every pitch is made up of $v$ voices, where each of our voices can have a value $v \in [0,128]$, where 0 represents silent.
\begin{figure}[!htb]
\centering
    \includegraphics[width=0.4\textwidth]{img/ds_transitionnaming.png}
    \caption{Transition naming}
      \label{dataset:trans}
\end{figure}
Generally this approach fails to capture held notes, the state of the art is using again a special symbol to represent when the previous pitch is held \cite{2019InpaintNet,datarepresentation}.
This approach however has as we have found out some shortcomings when used in our Model. An evaluation can be found in TODO:think about how to present this, here or later or somehow.
Therefor we used a novel approach to encode held notes such that for each pitch we additionally have a corresponding held note representation.
This leads us to our final encoding for one voice $v \in [0,256)$ i.e. the pitch C4 would be represented as $72$ and as $72+128=200$ if it is held.
Thus we can define a transition as
\begin{center}
    $x \in \{0,1,...,256\}^{12\times 16 \times v}$
\end{center}
\subsection{Preprocessing}
Since we wanted our model to learn vivid transitions we additionally filtered our transitions, based on the additional metrics presented in subsection \ref{sub:datasetMetrics}.
We filtered our transitions based on whether pitches start in the surrounding half-bars.
Only if all half-bars surrounding the TP have at least one non-silent pitch starting in it we consider the TP for our work.
All half-bars here refer to the respective 4 half-bars the Target is made up of.\\
The reasoning behind this is that we wanted to eliminate transition which consisted of long-held notes and or silent Transitions, to encourage the Model to generate vivid transitions.
After the filtering has been applied we additionally enforced all transitions to be in a 4/4 beat and have consistent tempo.\\
Since we wanted our model to generalize both over transposition and music in general we used two augmentation methods in this work.
\subsubsection{Horizontal Augmentation}
Horizontal augmentation is the process of taking our transition and shifting them by one bar.
This means we effectively move over a song and take each consecutive 12 bars as a transition.
This augmentation method was mostly used for pretraining to ensure our model first learn to generate music before it generates transitions.
\subsubsection{Vertical Augmentation}
Vertical augmentation is the process of taking our transitions and applying a transposition to each of them.
We transposed each transition 22 times, for each half-step for 11 half steps up and down.
This results in an augmentation of roughly 20 since for this process to work we need the highest pitch in the transition to be inside our maximum pitch range of 128.
This augmentation method was used for all training steps to ensure our model learns to generalize over transpositions.
\subsection{Datasets used}
A detailed list of all datesets we used for training and evaluation \ref{dataset:fin}.\\
\begin{table}[H]
\begin{tabular}{|l|l|l|l|l|}
\hline
                                                                                 & Bars & \begin{tabular}[c]{@{}l@{}}Vertical\\ Aug.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Horizontal\\ Aug.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Number of\\ Entries\end{tabular}    \\ \hline
1 Bar Dataset                                                                    & 1    & True                                                    & True                                                      & 7'966'272 \\ \hline
\begin{tabular}[c]{@{}l@{}}12 Bar Dataset \\ Pretrain\end{tabular}               & 12   & True                                                    & True                                                      & 663'856   \\ \hline
\begin{tabular}[c]{@{}l@{}}12 Bar Dataset \\ Finetune\end{tabular} & 12 & False & False                                                     & 4161 \\ \hline
\end{tabular}
    \caption{Overview of the data used, TODO: put all shapes and counts here we later on use to show anything, such as that held works etc.}
      \label{dataset:fin}
\end{table}


==> chapters/ch04-model.tex <==
\section{Model}
Our model extends the already existing InpaintNet presented by \cite{2019InpaintNet}. The model consists of a variational autoencoder (VAE) that maps our representation of the music bars to a latent space. In a second step, a generation RNN works on the latent space and generates the missing music bars given the pre and past context of the corresponding music piece.\\


\subsection{Modified MeasureVAE}
\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{img/model_vae.png}
    \caption{VAE based on the model of \cite{2019InpaintNet}, image extended from the one in their paper.}
    \label{fig:model_vae}
\end{figure}

The encoder consists of en embedding layer for each of the voices in the original measure. The following convolution layer with a kernel size of $(1,3)$ reduces the dimensions of the tensor by one. Like in the original model, this tensor is fed into a bidirectional RNN followed by two linear stacks to obtain the distribution to sample the latent vector $z$ from.\\
The beat-RNN of the decoder was left untouched, and the tick-RNN followed by the linear stack was multiplied to generate the different voices of the reconstructed music bar. There is no correspondence between the RNN's that generate the individual voices.

\subsection{Unchanged LatentRNN}


\textcolor{red}{The RNN that works on the latent space was left unchanged, do we just want to reference to the original paper or include an image?}

\subsection{Training}

During the training of the model, we insert four bars of pre- and past-context and inpaint four bars of music. In a first step, the MeasureVAE is trained for at least 30 epochs and learns to correctly reconstruct music from the latent space.\\
After this training, the weights of the MeasureVAE were freezed and we train the LatentRNN on our augmented pretrain dataset for 180 epochs followed by a finetune phase of another 50 epochs on our original transitions dataset.\\


==> chapters/ch05-metrics.tex <==
\section{Metrics}
In the current Music Deep Learning Community most projects are evaluated using user studies. 
Since for the development and tuning of Deep Learning Musik Generation Models(MGMs) a purely automatic set of metrics would increase the productivity we implemented the following set of metrics.
A python package that calculates them for a set of midis can be found at TODO: link.
\subsection{Dissonant Ratio}
To evaluate the harmonic properties of MGMs we prose to evaluate the distribution of Dissonant Intervals to consonant intervals.
We argue that the distribution of the generated music and the distribution of the original intervals should be ideally similar.
A high score in this metric will clearly indicate that the MGMs is producing unpleasant music.
We define the intervals Minor-Second, Triton, and Major-Seventh as dissonant intervals e.g. $\{1, 6, 11\}$. While other intervals depending on the period may also be considered dissonant, we found that this set of intervals is considered as dissonant in most works \cite{dis2,dis1,tritdis}.
To our best knowledge this metric is novel in the area of MGMs.
For intervals outside of the range of one octave, we defined this operation to be modulo 12,
\begin{center}
$$
isDissonant(x)=
\begin{cases}
1, if x \in \{1, 6, 11\}\\
0, else
\end{cases}
$$
\end{center}
Let the concurrently played pitches be a vector $x \in $\{1, 2,...,128\}$^v$, where v is the amount of voices.
Now the dissonant ratio is defined as
\begin{center}
    $DSR(x)=\frac{\sum_{i=1}^{v-1}\sum_{j=i+1}^{v}{isDissonant(|x[i]-x[j]| \mod 12)}}{\binom{v}{2}}$
\end{center}
in other words, it is the amount of dissonant interval combinations over the total amount of interval combinations.

\subsection{Silent Ratio}
Often in our process the MGM defaulted to predicting the most common pitch, the silent pitch.
This alone can not be detected by looking at the pitch accuracy.
A similar approach has already been defined by de Leon et al. \cite{evolutionaryComputation}.
We define the silent ratio qualitatively as the amount of silent notes divided by the amount of total notes.

\subsection{Variety Ratio-MAYBE CUT}
When working on a big range of pitches, such as our 128 pitch range, a undesirbale model may learn to predict a big range of pitches which does not appear like this in the original distribution.
We discovered that our Models are a lot richer in variety then the original distribution, which we consider to be undesirable.
To capture this aspect of development we defined the Variety score. Qualitatively it can be defined as the amount of used pitches over the total amount of possible pitches.

\subsection{Length Variety Ratio-MAY BE CHANGED}
Another issue that often arises is that the note length may not match with the human perception of music, i.e. random many short notes or mode collapse single very long held notes.
Therefore we define the ratio of held notes over the total amount of notes.
Let a song be defined as a sequence of voice combinations $x \in We should probably define this earlier in dataset$ 
Then we can define
$LVR(s)=\frac{AmountOfHeldNotes}{AmountOfNotes}$

\subsection{Variety Score-MAY BE CHANGED}

\begin{center}
$$
VarietyScore=\frac{AmountOfUniqueChords}{Length}
$$
\end{center}


==> chapters/ch06-results.tex <==
\section{Results}

\textcolor{red}{move this part up before the metrics part? because its the exact results and metrics is evaluation. But we also have a metrics chapter here ...}

\textcolor{red}{should we show the improvement in trainingstime when using augmented dataset?}

\subsection{Monophonic music generation}

When evaluating the original model and generating monophonic music, the model gets lost in predicting only held notes, because this class is by far the most common class in the dataset. Despite having a low loss and a high accuracy on the validation data, the predicted inpainted bars are not desired music. The generated bars often consist of very few notes that are held over multiple bars or even completely silent transitions.\textcolor{red}{confirm this! no changes in held seen from current evaluation, but we can find examples}\\
With our alternative encoding scheme, where we double the number of notes to encode each held note separately, the model achieves better predictions although the loss and accuracy is worse. This difference in the predicted music can also be seen in the evaluation in figure \ref{fig:improvement_held_approach_1v}.

\begin{figure}[H]
    \centering
    \includegraphics[height=8cm]{plots/rnn_1_improvement_held_approach.png}
    \caption{left: our approach, right: original approach, ratio of silent notes, other ideas to make this visible?}
    \label{fig:improvement_held_approach_1v}
\end{figure}

\subsection{Polyphonic music generation for 3 voices}

For the polyphonic music generation we use our proposed encoding to encode held notes with separate classes.\\
After the training of the modified MeasureVAE, we observe a reconstruction accuracy from the latent space to the complete representation for three voices of 96\%.\\
After freezing the weights of the VAE, we pretrain the LatentRNN for 180 epochs as seen in figure \ref{fig:rnn_pretrain_3V}. 


\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{plots/rnn_3_pretrain.png}
    \caption{probs switch to png bcs of template}
    \label{fig:rnn_pretrain_3V}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{plots/rnn_3_improvement_finetune.png}
    \caption{}
    \label{fig:rnn_finetune_3V}
\end{figure}

\begin{figure}[H]
    \fontsize{7}{10}\selectfont
    \centering
    \includesvg[width=\columnwidth]{plots/rnn_3_improvement_finetune.svg}
    \caption{this may work with a smaller legend}
    \label{fig:rnn_finetune_3V}
\end{figure}

\subsection{Metrics}
Evaluation with metrics here

\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{plots/metrics_results_1.png}
    \caption{metrics\_results\_1}
    \label{fig:metrics_results_1}
\end{figure}

some text here

\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{plots/metrics_results_2.png}
    \caption{metrics\_results\_2}
    \label{fig:metrics_results_2}
\end{figure}

==> chapters/ch07-discussion.tex <==
\section{Discussion}

==> img/inpaintpdf.tex <==
%% Creator: Inkscape inkscape 0.92.3, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'inpaint.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{397.69585512bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.45841164)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\textwidth,page=1]{inpaint.pdf}}%
    \put(0.46806806,0.26368113){\color[rgb]{0,0,0}\rotatebox{90}{\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Encoder\end{tabular}}}}}%
    \put(0,0){\includegraphics[width=\textwidth,page=2]{inpaint.pdf}}%
    \put(0.72005107,0.21356521){\color[rgb]{0,0,0}\rotatebox{-90}{\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Decoder\end{tabular}}}}}%
  \end{picture}%
\endgroup%

